An inverse boundary value problem arising in nonlinear acoustics

We consider an inverse problem arising in nonlinear ultrasound imaging. The propagation of ultrasound waves is modeled by a quasilinear wave equation. We make measurements at the boundary of the medium encoded in the Dirichlet-to-Neumann map, and we show that these measurements determine the nonlinearity.

==> construction_previous.tex <==



In the following, we use the notations 
\begin{align*}
C(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)}) 
&= \sum_{(i,j,k,l) \in \Sigma(4)} (4\frac{(\ziz + \zjz + \zkz)^2}{|\zi + \zj + \zk|^2_{g^*}} + \frac{(\ziz+\zlz)^2}{| \zi + \zl|^2_{g^*}})
\frac{(\zjz + \zkz)^2}{|\zeta^{(j)} + \zeta^{(k)}|^2_{g^*}},\\
%& \equiv C_1 + C_2 \nonumber \\
D(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)})  &=  \sum_{(i,j,k,l) \in \Sigma(4)} (3 \frac{(\zkz+\zlz)^2}{| \zk + \zl|^2_{g^*}} + 2\frac{(\ziz + \zjz + \zkz)^2}{|\zi + \zj + \zk|^2_{g^*}}).
%& \equiv D_1 + D_2 \nonumber 
\end{align*}
The above analysis shows that from the third order linearization of $\Lambda$, one can recover the quantity 
$-C \beta_2^3 + D \beta_2 \beta_3 - \beta_4$. 
We would like to show that for fixed $q$, we can find three different sets 
\[
(\zeta^{(1),k}, \zeta^{(2),k}, \zeta^{(3),k}, \zeta^{(4),k}), k = 1,2,3,
\] 
such that the vectors 
\[
(-C(\zeta^{(1),k}, \zeta^{(2),k}, \zeta^{(3),k}, \zeta^{(4),k}), D(\zeta^{(1),k}, \zeta^{(2),k}, \zeta^{(3),k}, \zeta^{(4),k}), -1),\ k=1,2,3,
\] are linearly independent. 
This implies that we can solve $\beta_2^3, \beta_2 \beta_3, \beta_4$ from a nondegenerate $3 \times 3$ linear system. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

First, we show that with ${\zh}^{(1)}$ satisfying $|\zh^{(1)}|_{g^*} = 1$ fixed, one can perturb it a little bit to choose $\zh^{(2)}, \zh^{(3)}, \zh^{(4)}$ such that $\zh^{(j)}, j=1,2,3,4$ are lightlike and linearly independent. 
For convenience, we form the lemma below based on the proof of  \cite[Lemma 3.5]{Kurylev2018}.
\begin{lm}\label{lm_perturb_y}
    Let $q \in I(p^-, p^+)$ and $\zh^{(1)} \in L^{*,+}_q M$ with $|\zh^{(1)}|_{g^*} = 1$. 
    Suppose there is $(x_1, \xi_1) \in L^{+} V$ with $(q, \zh^{(1)}) = (\gamma_{x_1, \xi_1}(t_1), (\dot{\gamma}_{x_1, \xi_1}(t_1))^b)$ and $0 < t_1 < \rho(x_1, \xi_1)$. 
    %satisfy $(q, w_o) = (\gamma_{z_o, \nu_o}(t_q),\dot{\gamma}_{z_o, \nu_o}(t_q))$ with $0 < t_q< \rho(z_o, \nu_o)$. 
    Then we can find  $\varsigma >0$ such that for any $\zh^{(2)} \in N^+(\zh^{(1)}, \varsigma)$, there exists a vector 
    $(x_2, \xi_2) \in L^{+} V$ with $(q, \zh^{(2)}) = (\gamma_{x_2, \xi_2}(t_2), (\dot{\gamma}_{x_2, \xi_2}(t_2))^b)$ and $0 < t_2 < \rho(x_2, \xi_2)$. 
    Moreover, one has $(x_1, \xi_1)$ and $(x_2, \xi_2)$ are causally independent. 
\end{lm}
\begin{proof}
    First set $w_1 = (\zh^{(1)})^\#$. 
    Note that the geodesic $\gamma_{q, -w_1}(t) = \gamma_{x_1, \xi_1}(t_1-t)$ have no cut points for $t \in [0, t_1]$, which implies $t_1 <  \rho(q, -w_1)$. 
    
    We consider all the null geodesics $\gamma_{q, -w}(t)$ that emanate from $q$ in the lightlike direction of $w$, where $w \in N^+(w_1, \varsigma)$ with $\varsigma$ to be specified later. 
    By \cite[Theorem 9.33]{Beem1996}, the cut locus function $\rho(q, -w_1)$ is lower semi-continuous on a globally hyperbolic Lorentzian manifold. 
    It follows that there is $\varsigma >0 $ such that $t_1 < \rho(q, -w)$ for any $w \in N^+(w_1, \varsigma)$.    
    Next, to find $(x_2, \xi_2) \in L^+V$ for such $(q, w)$, 
    let $\gamma_{q, -w}(t_x)$ be the intersection points of $\gamma_{q, -w}$ with the Cauchy surface $\{x \in M: \textbf{t}(x) = \textbf{t}(x_1)\}$, where $\textbf{t}$ is the time function on $(M, g)$. 
    Indeed, the first cut point comes at or before the first conjugate point along $\gamma_{q, -w_1}(t)$. 
    This implies the exponential map is a local diffeomorphism near $-t_1 w_1 \in L^-_q M$, which maps a small neighborhood of $-t_1 w_1$ to a small neighborhood of $x_1$.  
    For $w$ close enough to $w_1$, there exist $t_x < t_1 + \epsilon < \rho(q, -w)$ and $x_2 = \gamma_{q,-w}(t_x) \in V$ with $\textbf{t}(x_2) = \textbf{t}(x_1)$, 
    for sufficiently small $\ep>0$. 
    %    By the inverse function theorem, such $t_y$ exists with $t_y < t_o + \epsilon < \rho(q, w)$ and $y \in U$, 
    %    for sufficiently small $\ep>0$ and $w$ close enough to $w_o$.   
    This proves the statement. 
\end{proof}
Now we choose local coordinates $x = (x^1, x^2, x^3, x^4)$ at $q$ such that $g$ coincides with the Mankowski metric. 
By rotating the coordinate system in the spatial variable, without loss of generality, we can assume
\[
\zeta = (-1, 0, \cos \varphi, \sin \varphi), \quad {\zh}^{(1)} = (-1, 1, 0, 0), 
\]
where $\varphi \in [0, 2\pi)$. For $\theta$ sufficiently small, we choose 
\begin{align*}
\zh^{(2)} &= (-1, \cos \theta, \sin \theta \sin \varphi, -\sin \theta \cos \varphi), \\
 \zh^{(3)} &= (-1, \cos \theta, -\sin \theta \sin \varphi, \sin \theta \cos \varphi), \\
\zh^{(4)} &=(-1, \cos \theta, \sin \theta \cos \varphi, \sin \theta \sin \varphi). 
\end{align*}
Then we have $\zeta = \sum_{j=1}^4 \zeta^{(j)}$, where we set $\zeta^{(j)} = \alpha_j \zh^{(j)}$ with
\begin{align*}
\alpha_1 = \frac{\cos \theta}{\cos \theta -1} , \quad \alpha_2 = \alpha_3= -\frac{(\cos \theta -1) + \sin \theta}{2(\cos \theta - 1) \sin \theta}, \quad \alpha_4 =  \frac{1}{\sin \theta}. 
\end{align*}
Let $\lambda = (\cos \theta - 1) \sin \theta$ and $a_j = {\alpha_j}/{\lambda}$, i.e.,
\begin{align*}
a_1 = {\cos \theta}\sin \theta , \quad \alpha_2 = \alpha_3= -\frac{(\cos \theta -1) + \sin \theta}{2}, \quad \alpha_4 = \cos \theta - 1 . 
\end{align*}
Note $\zeta_0^{(j)} = \alpha_j, j = 1, 2,3, 4$. 
We compute
\[
| \zk + \zl|^2_{g^*} = 2 \lge \zk, \zl \rge_{g^*} = 2 \alpha_k \alpha_l \lge \zh^{(k)}, \zh^{(l)} \rge_{g^*},
\]
and 
\begin{align*}
&| \zeta^{(1)} + \zeta^{(2)}|^2_{g^*} = 2 \alpha_1\alpha_2 (\cos \theta - 1),   
&| \zeta^{(1)} + \zeta^{(3)}|^2_{g^*} = 2 \alpha_1\alpha_3(\cos \theta - 1), \\
&| \zeta^{(1)} + \zeta^{(4)}|^2_{g^*} = 2 \alpha_1\alpha_4(\cos \theta - 1),  
&| \zeta^{(2)} + \zeta^{(3)}|^2_{g^*} = -4\alpha_2 \alpha_3 \sin^2 \theta, \\
&| \zeta^{(2)} + \zeta^{(4)}|^2_{g^*} = -2\alpha_2 \alpha_4 \sin^2 \theta, 
&| \zeta^{(3)} + \zeta^{(4)}|^2_{g^*} = -2\alpha_3 \alpha_4 \sin^2 \theta, 
\end{align*}
It follows that
\begin{align*}
&\frac{(\zeta_0^{(1)} + \zeta_0^{(2)})^2}{| \zeta^{(1)} + \zeta^{(2)}|^2_{g^*}}  = \frac{(\alpha_1 + \alpha_2)^2}{2 \alpha_1\alpha_2 (\cos \theta - 1)} 
\equiv \frac{1}{2(\cos \theta -1)}I_1,\\ 
&\frac{(\zeta_0^{(1)} + \zeta_0^{(3)})^2}{| \zeta^{(1)} + \zeta^{(3)}|^2_{g^*}}  = \frac{(\alpha_1 + \alpha_3)^2}{2 \alpha_1\alpha_3 (\cos \theta - 1)}
\equiv \frac{1}{2(\cos \theta -1)}I_1, \\
&\frac{(\zeta_0^{(1)} + \zeta_0^{(4)})^2}{| \zeta^{(1)} + \zeta^{(4)}|^2_{g^*}}  = \frac{(\alpha_1 + \alpha_4)^2}{2 \alpha_1\alpha_4 (\cos \theta - 1)} 
\equiv \frac{1}{2(\cos \theta -1)}I_3, \\
&\frac{(\zeta_0^{(2)} + \zeta_0^{(3)})^2}{| \zeta^{(2)} + \zeta^{(3)}|^2_{g^*}}  
= \frac{(\alpha_2 + \alpha_3)^2}{-4\alpha_2 \alpha_3 \sin^2 \theta} 
= -\frac{1}{\sin^2 \theta}, \\
&\frac{(\zeta_0^{(2)} + \zeta_0^{(4)})^2}{| \zeta^{(2)} + \zeta^{(4)}|^2_{g^*}}  = \frac{(\alpha_2 + \alpha_4)^2}{-2\alpha_2 \alpha_4 \sin^2 \theta}
\equiv -\frac{1}{2\sin^2 \theta}I_2,\\
&\frac{(\zeta_0^{(3)} + \zeta_0^{(4)})^2}{| \zeta^{(3)} + \zeta^{(4)}|^2_{g^*}}  = \frac{(\alpha_3 + \alpha_4)^2}{-2\alpha_3 \alpha_4 \sin^2 \theta}
\equiv -\frac{1}{2\sin^2 \theta}I_2,
\end{align*}
where we write $s = \sintw$ and compute 
\begin{align*}
I_1 &= \frac{(\alpha_1 + \alpha_2)^2}{\alpha_1\alpha_2 }
= -\frac{1}{2 \cos \theta} + (-2 \costw + \frac{1}{2 \costw \costt})s + 2s^2,\\
%&= \frac{1}{\costw \cos \theta}( -\frac{\costw}{2} + \sintw(-2\cos \theta + \frac{1}{2}) + 2 \sin^2 \thett (2 \costw \cos \theta) + \sin^3 \thett(2 \costt)),\\
I_2 &= \frac{(\alpha_2 + \alpha_4)^2}{\alpha_2\alpha_4 }
= (\frac{\costw}{2})\frac{1}{s} +\frac{3}{2} + 2 \costw s + 2 s^2 +  (-\frac{4}{\sintw - \costw}) s^3,\\
I_3 &= \frac{(\alpha_1 + \alpha_4)^2}{\alpha_1\alpha_4 }
= (-\costw \cos \theta) \frac{1}{s}+ 2 + (-\frac{1}{\costw\cos \theta})s.
\end{align*}
Here we expand each term according to the order of $s$. 
Note that $(\costw \cos\theta) I_1$, $(s\cos \theta )I_2$, $(s\costw \cos \theta )I_3$ are real analytic functions. 
Then we compute
\begin{align*}
D_1(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)})  &=  \sum_{(i,j,k,l) \in \Sigma(4)} 3 \frac{(\zkz+\zlz)^2}{| \zk + \zl|^2_{g^*}}\\
& = 3 \times 4 (\frac{1}{\cos \theta -1} I_1 + \frac{1}{2(\cos \theta -1)}I_3 - \frac{1}{\sin^2\theta} + \frac{1}{\sin^2 \theta}I_2)\\
& =\frac{3}{(\costt +1)s^3}(-\costw \cos \theta + 7 s + \mathcal{O}(s^2)). 
\end{align*}
Since for $(i,j,k,l) \in \Sigma(4)$ we have
\[
|\zj + \zk + \zl|^2_{g^*} = |\zeta - \zi|^2_{g^*} = -2 \alpha_i \lge \zeta, \zh^{(i)} \rge_{g^*},
\]
then 
\begin{align*}
&| \zeta^{(1)} + \zeta^{(2)}+ \zeta^{(3)}|^2_{g^*} 
= -2 \alpha_4(\sin \theta -1), 
&| \zeta^{(1)} + \zeta^{(2)}+ \zeta^{(4)}|^2_{g^*} 
= 2\alpha_3,\\
&| \zeta^{(1)} + \zeta^{(3)}+ \zeta^{(4)}|^2_{g^*} 
= 2\alpha_2,
&| \zeta^{(2)} + \zeta^{(3)}+ \zeta^{(4)}|^2_{g^*} 
= 2\alpha_1. 
\end{align*}
We compute
\begin{align*}
&R_{123} \equiv \frac{(\zeta_0^{(1)} + \zeta_0^{(2)}+ \zeta_0^{(3)})^2}{| \zeta^{(1)} + \zeta^{(2)}+ \zeta^{(3)}|^2_{g^*}}  = \frac{(1-\alpha_4)^2}{-2 \alpha_4(\sin \theta -1)}
=\frac{1-\sin\theta}{2\sin \theta} = -\frac{1}{2} + \frac{1}{4 \costw} s,\\
&R_{124} \equiv \frac{(\zeta_0^{(1)} + \zeta_0^{(2)}+ \zeta_0^{(4)})^2}{| \zeta^{(1)} + \zeta^{(2)}+ \zeta^{(4)}|^2_{g^*}}  = \frac{(1-\alpha_3)^2}{2\alpha_3}
= -\frac{1}{4}(\frac{1}{\sin \theta} + \frac{1}{\cos \theta -1}) -1 -\frac{(\cos \theta -1 )\sin \theta}{(\cos \theta -1 ) + \sin \theta}\\
& \quad \quad \quad \quad \quad \quad  \quad \quad \quad \quad \quad \quad=  \frac{1}{8s^2} - \frac{1}{8 \costw} \frac{1}{s} -1 + (1 + \frac{1}{\costt}) s^2 + (\frac{2\costw}{\costt})s^3,
\\
&R_{134} \equiv \frac{(\zeta_0^{(1)} + \zeta_0^{(3)}+ \zeta_0^{(4)})^2}{| \zeta^{(1)} + \zeta^{(3)}+ \zeta^{(4)}|^2_{g^*}}  = \frac{(1-\alpha_2)^2}{2\alpha_2}
= R_{124}, \\
&R_{234} \equiv \frac{(\zeta_0^{(2)} + \zeta_0^{(3)}+ \zeta_0^{(4)})^2}{|\zeta^{(2)} + \zeta^{(3)}+ \zeta^{(4)}|^2_{g^*}}  = \frac{(1-\alpha_1)^2}{2 \alpha_1}
=\frac{1}{2 \cos \theta(\cos \theta -1)} = -\frac{1}{4 \costt} \frac{1}{s^2}.
\end{align*}
Note that $s\costw R_{123}$, $s^2\costw \costt R_{124}$, $s^2\costw \costt R_{134}$, $s^2 \costt R_{234}$ are real analytic functions. 
Then we have 
\begin{align*}
D_2(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)})  
&=  \sum_{(i,j,k,l) \in \Sigma(4)}  2\frac{(\ziz + \zjz + \zkz)^2}{|\zi + \zj + \zk|^2_{g^*}} = (\frac{1}{2} - \frac{1}{2 \costt})\frac{1}{s^2} + \mathcal{O}(\frac{1}{s}).
%& = \frac{3}{s^2}(-\frac{1}{\costt} + \frac{1}{\costw} s + (8 R_{124} -2)s^2)
\end{align*}
This implies 
\begin{align*}
d(\theta) \equiv D(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)})  
&= \frac{3}{(\costt +1)s^3}(-\costw \cos \theta + \mathcal{O}(s)).
\end{align*}
Next, we compute
\begin{align*}
&C_2(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)})   
= \sum_{(i,j,k,l) \in \Sigma(4)} \frac{(\ziz+\zlz)^2}{| \zi + \zl|^2_{g^*}}
\frac{(\zjz + \zkz)^2}{|\zeta^{(j)} + \zeta^{(k)}|^2_{g^*}}\\
=& \frac{4}{(\cos \theta -1)^2(\costt +1)}(I_1 I_2 + I_3)\\
=& -\frac{1}{(\costt +1)s^4}((-\frac{\costw}{4 \costt} - \costw \costt)\frac{1}{s} \\
&+ (1 - \frac{1}{2 \costt}) + (-2\costw - \frac{1}{4\costw \costt} - \frac{\costw}{\costt})s + \mathcal{O}(s^2)). 
\end{align*}
We have 
\begin{align*}
&C_1(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)})   
= \sum_{(i,j,k,l) \in \Sigma(4)} 4\frac{(\ziz + \zjz + \zkz)^2}{|\zi + \zj + \zk|^2_{g^*}}
\frac{(\zjz + \zkz)^2}{|\zeta^{(j)} + \zeta^{(k)}|^2_{g^*}}
%=& 4 (R_{123}(\frac{1}{(\cos \theta -1)}I_1 -\frac{1}{4\sin^2 \theta}) + 2 R_{124} (\frac{1}{2(\cos \theta -1)}(I_1 + I_3)-\frac{1}{2\sin^2 \theta} ) ) \\
%&+ R_{234}( \frac{1}{-4\sin^\theta}(1+4I_2))
=  4 (C_{11} + C_{12} + C_{13}),
\end{align*}
where 
\begin{align*}
C_{11} &= \frac{(\zeta_0^{(1)} + \zeta_0^{(2)}+ \zeta_0^{(3)})^2}{| \zeta^{(1)} + \zeta^{(2)}+ \zeta^{(3)}|^2_{g^*}}
(\frac{(\zeta_0^{(1)} + \zeta_0^{(2)})^2}{| \zeta^{(1)} + \zeta^{(2)}|^2_{g^*}} 
+ \frac{(\zeta_0^{(1)} + \zeta_0^{(3)})^2}{| \zeta^{(1)} + \zeta^{(3)}|^2_{g^*}}
+\frac{(\zeta_0^{(2)} + \zeta_0^{(3)})^2}{| \zeta^{(2)} + \zeta^{(3)}|^2_{g^*}}
) \\
&= R_{123}(\frac{1}{(\cos \theta -1)}I_1 -\frac{1}{4\sin^2 \theta}) 
= R_{123}(\frac{1}{-2s^2}I_1 -\frac{1}{8\costw}\frac{1}{s})\\
& =  -\frac{1}{4(\costt +1)s^4}(3 \costw s^2 + \mathcal{O}(s^3)),
\end{align*}
and
\begin{align*}
C_{12} &= \frac{(\zeta_0^{(1)} + \zeta_0^{(2)}+ \zeta_0^{(4)})^2}{| \zeta^{(1)} + \zeta^{(2)}+ \zeta^{(4)}|^2_{g^*}}
(\frac{(\zeta_0^{(1)} + \zeta_0^{(2)})^2}{| \zeta^{(1)} + \zeta^{(2)}|^2_{g^*}} 
+ \frac{(\zeta_0^{(1)} + \zeta_0^{(4)})^2}{| \zeta^{(1)} + \zeta^{(4)}|^2_{g^*}}
+\frac{(\zeta_0^{(2)} + \zeta_0^{(4)})^2}{| \zeta^{(2)} + \zeta^{(4)}|^2_{g^*}}
) \\
&= 2 R_{124} (\frac{1}{2(\cos \theta -1)}(I_1 + I_3)-\frac{1}{2\sin^2 \theta}I_2 ) \\
& =  -\frac{1}{4(\costt +1)s^4}((\frac{3}{4\costw})\frac{1}{s} + (-\frac{7}{2} + \frac{1}{\costt}) \\
&+ (\frac{11}{4\costw} - \costw \costt - 7 \costw)s + \mathcal{O}(s^2))
\end{align*}
and
\begin{align*}
C_{13}  &= \frac{(\zeta_0^{(2)} + \zeta_0^{(3)}+ \zeta_0^{(4)})^2}{| \zeta^{(2)} + \zeta^{(3)}+ \zeta^{(4)}|^2_{g^*}}
(\frac{(\zeta_0^{(2)} + \zeta_0^{(3)})^2}{| \zeta^{(2)} + \zeta^{(3)}|^2_{g^*}} 
+ \frac{(\zeta_0^{(3)} + \zeta_0^{(4)})^2}{| \zeta^{(3)} + \zeta^{(4)}|^2_{g^*}}
+\frac{(\zeta_0^{(2)} + \zeta_0^{(4)})^2}{| \zeta^{(2)} + \zeta^{(4)}|^2_{g^*}}
) \\ 
&= R_{234}( \frac{1}{-\sin^2\theta}(1+I_2))\\
& =  -\frac{1}{4(\costt +1)s^4}(\frac{\costw}{2\costt}\frac{1}{s} + \frac{5}{2\costt} + \frac{2\costw}{\costt}s + \frac{2}{\costt} s^2). 
\end{align*}
It follows that 
\begin{align*}
C_1(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)})   
=& -\frac{1}{(\costt +1)s^4}((\frac{3}{4\costw} +\frac{\costw}{2\costt} )\frac{1}{s} 
+ (-\costw \costt +\frac{5}{2\costt} )\\
&+ (\frac{11}{4\costw} - \costw \costt - 7 \costw + \frac{2\costw}{\costt})s
+  \mathcal{O}(s^2).
)
\end{align*}
Then we have 
\begin{align*}
&c(\theta) \equiv  C(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)}) \\
=&  -\frac{1}{(\costt +1)s^4}((-\frac{\costw}{4 \costt} - \costw \costt + \frac{3}{4\costw} +\frac{\costw}{2\costt}
)\frac{1}{s} \\
&+ (1 - \frac{1}{2 \costt} -\costw \costt +\frac{5}{2\costt} ) \\
%+ (-2\costw - \frac{1}{4\costw \costt} - \frac{\costw}{\costt} \\
%&+ \frac{11}{4\costw} - \costw \costt - 7 \costw + \frac{2\costw}{\costt})s + \mathcal{O}(s^2)).
&+ (-9\costw - \frac{1}{4\costw \costt} + \frac{\costw}{\costt} 
+ \frac{11}{4\costw} - \costw \costt)s + \mathcal{O}(s^2)).
\end{align*}
Note that 
\begin{align*}
(-\frac{\costw}{4 \costt} - \costw \costt + \frac{3}{4\costw} +\frac{\costw}{2\costt})\frac{1}{s} 
&= (\frac{\cos \thett}{\cos \theta} + \frac{3}{2} \costw)s - \frac{1}{\costt} s^3,\\
1 - \frac{1}{2 \costt} -\frac{7}{2} + \frac{1}{\costt} +\frac{5}{2\costt}  &= \frac{5 s^2}{\cos \theta}. 
\end{align*}
Thus, we have 
\begin{align*}
&c(\theta) = C(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)}) 
=  -\frac{1}{(\costt +1)s^3}
((-\frac{15}{2}\costw +  \\
&\quad \quad \quad - \frac{1}{4\costw \costt} + \frac{2\costw}{\costt} 
+ \frac{11}{4\costw} - \costw \costt)) ) + \mathcal{O}(\frac{1}{s^2}). 
\end{align*}

This implies that 
\begin{align}\label{eq_limitcd}
\lim_{\theta \rightarrow 0} \frac{C(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)}) }{D(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)}, \zeta^{(4)}) }
 = -\frac{4}{3}. 
\end{align}
\begin{lm}
%The functions $ (\sin^3 \thett \cos^3 \thett \cos^2\theta) c(\theta)$ and $(\sin^3 \thett  \cos^3 \thett \cos^2\theta) d(\theta)$ are real analytic. 
There do not exist $k \in \mathbb{R}$ and $\ep > 0$ such that $c(\theta) = k d(\theta)$ for any $\theta \in (0, \ep)$. 
Then we can choose sufficiently small $\theta_1, \theta_2, \theta_3 > 0 $ such that
\[
(c(\theta_j), -d(\theta_j), 1), \quad j=1,2,3,
\]
are linearly independent. 
\end{lm}
\begin{proof}
We prove by contradiction. 
Assume there exists such $k$ and $\ep >0$.
By (\ref{eq_limitcd}), we must have $k = -\frac{4}{3}$. 
Then for $\theta \in (0, \ep)$, one has 
\[
3 c(\theta) + 4 d(\theta) \equiv 0.\]
Note that  $ (\sin^3 \thett \cos^2 \thett \cos^2\theta) c(\theta)$ and $(\sin^3 \thett  \cos^2 \thett \cos^2\theta) d(\theta)$ are real analytic functions. 
It follows that \[h(\theta) = (\sin^3 \thett \cos^3 \thett \cos^2\theta) (3 c(\theta) + 4 d(\theta))\] are real analytic. 
Since $h(\theta)$ vanishes in an open interval, it must vanish for all $\theta \in \mathbb{R}$. 
Now consider $\theta = {\pi}/{3}$. 
A straightforward computation shows that 
\begin{align*}
&\frac{(\zeta_0^{(1)} + \zeta_0^{(2)})^2}{| \zeta^{(1)} + \zeta^{(2)}|^2_{g^*}}  = 0, \quad 
&\frac{(\zeta_0^{(1)} + \zeta_0^{(3)})^2}{| \zeta^{(1)} + \zeta^{(3)}|^2_{g^*}}  = 0, \quad 
&\frac{(\zeta_0^{(1)} + \zeta_0^{(4)})^2}{| \zeta^{(1)} + \zeta^{(4)}|^2_{g^*}}  = -\frac{9}{\sqrt{2}} - 2\sqrt{2}, \\
&\frac{(\zeta_0^{(2)} + \zeta_0^{(3)})^2}{| \zeta^{(2)} + \zeta^{(3)}|^2_{g^*}}  = -2, \quad 
&\frac{(\zeta_0^{(2)} + \zeta_0^{(4)})^2}{| \zeta^{(2)} + \zeta^{(4)}|^2_{g^*}}  = 1-\frac{\sqrt{2}}{2}, \quad 
&\frac{(\zeta_0^{(3)} + \zeta_0^{(4)})^2}{| \zeta^{(3)} + \zeta^{(4)}|^2_{g^*}}  = 1-\frac{\sqrt{2}}{2},
\end{align*}
and 
\begin{align*}
&R_{123} = -\frac{\sqrt{2}}{2} - \frac{1}{2}, \quad 
&R_{124} = R_{134} = \sqrt{2}-1, \quad 
&R_{234} = -\sqrt{2} - 1. 
\end{align*}
Thus, we have
\begin{align*}
&D_1 = -54 -36 \sqrt{2}, \quad 
&D_2 = 6\sqrt{2} - 42, \quad 
&C_1 = 0, \quad 
&C_2 = 72 + 32 \sqrt{2}, 
\end{align*}
which implies that 
\begin{align*}
h(-\pi/4) = \frac{1}{2}\sin^3 (\pi/8) \cos^2 (\pi/8) (-168-24\sqrt{2}) \neq 0.
\end{align*}
This contradicts with $h(\theta) \equiv 0$. 
Therefore, such $k$ and $\ep$ do not exist. 


It follows that $g(\theta) \equiv  c(\theta) + \frac{4}{3} d(\theta)$ does not vanish in any open interval near $\theta = 0$. 
Note that $g(\theta)$ is smooth near $\theta = 0$ and $\lim_{\theta \rightarrow 0} (\sin^3 \thett {g(\theta)}) = 0$. 
In particular, 
by previous computation, one can show that there exist constants $a, b$ such that 
\[
%\frac{a}{\sintw} < |g(\theta)| < \frac{a}{\sin^2 \thett}
a < |g(\theta)| < \frac{b}{\sin^2 \thett}
\]
for $\theta$ small enough. 
%Then we can find different $\theta_j, j=1,2,3$ in a small neighborhood of $\theta = 0$, such that
%\begin{align*}
%\frac{c(\theta_1)}{d(\theta_1)} = -\frac{4}{3} + r, \quad 
%\frac{c(\theta_2)}{d(\theta_2)} = -\frac{4}{3} + 2r, \quad 
%\frac{c(\theta_3)}{d(\theta_3)} = -\frac{4}{3} + 4r,
%\end{align*}
%with $|r| > 0$ small enough. 
In the following, we would like to find $\theta_j, j=1,2,3$ in a small neighborhood of $\theta = 0$, such that the determinant does not vanish, i.e., 
\begin{align*}
&\det
\left[ {
    \begin{array}{ccc}
    c(\theta_1) & d(\theta_1) & 1 \\
    c(\theta_2) & d(\theta_2) & 1 \\
    c(\theta_3) & d(\theta_3) & 1 
    \end{array} 
} \right] \neq 0
\end{align*}
For simplification, we write $g(\theta_j) = g_j$ and $d(\theta_j) = d_j$ for $j = 1,2,3$. 
We compute
\begin{align*}
&\det
\left[ {
    \begin{array}{ccc}
    c(\theta_1) & d(\theta_1) & 1 \\
    c(\theta_2) & d(\theta_2) & 1 \\
    c(\theta_3) & d(\theta_3) & 1 
    \end{array} 
} \right]
%=
%\det
%\left[ {
%    \begin{array}{ccc}
%    g(\theta_1) & d(\theta_1) & 1 \\
%    g(\theta_2) & d(\theta_2) & 1 \\
%    g(\theta_3) & d(\theta_3) & 1 
%    \end{array} 
%} \right]\\
%& = (g(\theta_2)d(\theta_3) - g(\theta_3)d(\theta_2)) - (g(\theta_1)d(\theta_3) - g(\theta_3)d(\theta_1)) + (g(\theta_1)d(\theta_2) - g(\theta_2)d(\theta_1))\\
%&= (g(\theta_2) - g(\theta_3))(d(\theta_1)- d(\theta_2)) + (g(\theta_1) - g(\theta_2))(d(\theta_3) - d(\theta_2)
=
\det
\left[ {
    \begin{array}{ccc}
    g_1 & d_1& 1 \\
    g_2 & d_2 & 1 \\
    g_3 & d_3 & 1 
    \end{array} 
} \right]\\
& = (g_2 d_3 - g_3 d_2) - (g_1 d_3 - g_3 d_1) + (g_1 d_2 - g_2 d_1)\\
&= (g_2 - g_3)(d_3- d_1) + (g_1 - g_2)(d_2 - d_3). 
\end{align*}
We choose sufficiently small $\theta_1$ with  
$
\sin \theta_2 = \frac{1}{r} \sin \theta_1, \sin \theta_3 =\frac{1}{r^2} \sin \theta_1
$
for large parameter $r > 1$. 
Let $t = \sin (\theta_1/2)$. 
One has 
\begin{align*}
&d_2 = - \frac{3}{ 2\sin^3 (\theta_2/2)} + \mathcal{O}(\frac{1}{ \sin^2 (\theta_2/2)}) 
= - \frac{3 r^3}{ 2t^3} + \mathcal{O}(\frac{r^2}{ t^2}), \\
&d_3 = - \frac{3}{ 2\sin^3 (\theta_3/2)} + \mathcal{O}(\frac{1}{ \sin^2 (\theta_3/2)}) 
= - \frac{3 r^6}{ 2t^3} + \mathcal{O}(\frac{r^4}{ t^2}),\\
& a < |g_2| < \frac{b}{\sin^2 (\theta_2/2)} = \frac{b r^2}{ t^2}, \quad 
a < |g_3| < \frac{b}{\sin^2 (\theta_3/2)} = \frac{b r^4}{ t^2}. 
\end{align*}
This implies that 
\begin{align*}
& d_3 - d_1 = - \frac{3 r^6}{ 2t^3} + \mathcal{O}(\frac{r^4}{ t^2} + \frac{1}{ t^3}), \quad 
&d_2 - d_3 = - \frac{3 r^6}{ 2t^3} + \mathcal{O}(\frac{r^4}{ t^2} + \frac{1}{ t^3}),\\
& 0 <|g_2 - g_3| <  \frac{b r^4}{ t^2}, \quad 
&0 <  |g_1 - g_2| < \frac{b r^2}{ t^2}. 
\end{align*}
Thus, we have 
\begin{align*}
(g_2 - g_3)(d_3- d_1) + (g_1 - g_2)(d_2 - d_3) = 
\end{align*}

\end{proof}

\newpage


==> linearization_Gaussian.tex <==
Nonlinear ultrasound waves are widely used in medical imaging. 
The propagation of high intensity ultrasound is described by nonlinear acoustic equations. 
More explicitly, let $\Omega$ be a bounded domain with smooth boundary in $\Rthree$.
Let $c(x) > 0$ be the wave speed and $\ptx$ denotes the pressure field. 
We consider 
\begin{equation}\label{eq_problem}
\begin{aligned}
\frac{1}{c^2(x)} \partial_t^2 \ptx  - \Delta \ptx  - F(x, p) &= 0, & \  & \mbox{in } (0,T) \times \Omega,\\
\ptx &= f, & \ &\mbox{on } (0,T) \times \partial \Omega,\\
p = {\partial_t p} &= 0, & \  & \mbox{on } \{t=0\},
\end{aligned}
\end{equation}
where $f$ is the isolation profile on the boundary and $F(x,p)$ is the nonlinear term. 
The measurement is the Dirichlet-to-Neumann (DN) map given by 
\[
\Lambda f = \partial_\nu p|_{(0, T) \times \partial \Omega},
\]
where $\nu$ is the outer unit normal vector to $\partial \Omega$. 


When $F(x,p) = \beta(x) \partial_t^2 (p^2)$, this equation is called Westervelt type 
and the recovery of 
$\beta(x)$ from the DN map is studied in \cite{ultra21} using the second order linearization and Gaussian beams.
This Westervelt equation can be regarded as a lower order approximation to a more complicated physical model, see \cite{Kaltenbacher2021}. 
In this project, we consider the more general nonlinear term 
\[
F(x,p) = \sum_{m=1} \beta_m(x) \partial_t^2 (p^{m+1}),
\]
with $\beta_m(x)$ smooth. 
We plan to study the recovery of the nonlinear coefficient $\beta_m(x)$ from the DN map. 

First, let $\ptx$ solve (\ref{eq_problem}) with $f = \sum_{j=1}^N \ep_j f_j$. 
Consider the solution $u_j$ to the linear wave equation with boundary source $f_j$, for $j=1,2, \ldots, N$, i.e.,
\begin{equation*}%\label{eq_problem}
\begin{aligned}
\frac{1}{c^2(x)} \partial_t^2 \ujtx - \Delta \ujtx  &= 0, & \  & \mbox{in } (0,T) \times \Omega,\\
\ujtx &= f_j, & \ &\mbox{on } (0,T) \times \partial \Omega,\\
\ujtx = {\partial_t \ujtx} &= 0, & \  & \mbox{on } \{t=0\}.
\end{aligned}
\end{equation*}
%and the solution to the backward wave equation with boundary source $f_0$, i.e.,
%\begin{equation*}%\label{eq_problem}
%\begin{aligned}
%\frac{1}{c^2(x)} \partial_t^2 u_0(t,x) - \Delta u_0(t,x)  &= 0, & \  & \mbox{in } (0,T) \times \Omega,\\
%u_0(t,x) &= f_0, & \ &\mbox{on } (0,T) \times \partial \Omega,\\
%u_0(t,x) = {\partial_t u_0(t,x)} &= 0, & \  & \mbox{on } \{t=0\}. 
%\end{aligned}
%\end{equation*}
Now we define 
\[
\UN = \epspN,
\]
and $\UN$ solves
\begin{equation}\label{eq_UN}
\begin{aligned}
\frac{1}{c^2(x)} \partial_t^2 \UN - \Delta \UN  - B_N(\beta_1, \ldots, \beta_{N-1}; u_1, \ldots, u_N) &= 0, & \  & \mbox{in } (0,T) \times \Omega,\\
\UN &= 0, & \ &\mbox{on } (0,T) \times \partial \Omega,\\
\UN = {\partial_t \UN} &= 0, & \  & \mbox{on } \{t=0\},
\end{aligned}
\end{equation}
where $B_N$ can be described in a inductive procedure below. 
When $N=2$, we write
\[
B_2(\beta_1; u_1, u_2) = \sum_{(i,j) \in \sigma(2)} \beta_1(x) \partial_t^2 (p_ip_j) = 2 \beta_1(x) \partial_t^2 (u_1u_1),
\]
where $\sigma(m)$ denotes the permutation of $\{1,2, \ldots, m\}$. 
Let $\mathcal{U}^{(2)}_{ij}$ solve (\ref{eq_UN}) with the nonlinear term $\beta_1(x) \partial_t^2 (p_ip_j)$ instead of $B_N$. 
When $N=3$, we can write
\begin{align*}
B_3(\beta_1,\beta_3; u_1, u_2, u_3) &= \sum_{(i,j,k) \in \sigma(3)} \beta_1(x) \partial_t^2 (\mathcal{U}^{2}_{ij}p_k) + \beta_2(x) \partial_t^2 (u_iu_ju_k) \\
&\equiv R_2(\beta_1; u_1, u_2, u_3) + 3! \beta_2(x) \partial_t^2 (u_1u_2u_3). 
\end{align*}
Then for general $N$, we can expect 
\[
B_N(\beta_1, \ldots, \beta_{N-1}; u_1, \ldots, u_N) = R_N(\beta_1, \ldots, \beta_{N-2}; u_1, \ldots, u_N) + N! \beta_{N-1}(x) \partial_t^2 (u_1u_2 \ldots u_N). 
\]

Consider the solution to the backward wave equation with boundary source $f_0$, i.e.,
\begin{equation*}%\label{eq_problem}
\begin{aligned}
\frac{1}{c^2(x)} \partial_t^2 u_0(t,x) - \Delta u_0(t,x)  &= 0, & \  & \mbox{in } (0,T) \times \Omega,\\
u_0(t,x) &= f_0, & \ &\mbox{on } (0,T) \times \partial \Omega,\\
u_0(t,x) = {\partial_t u_0(t,x)} &= 0, & \  & \mbox{on } \{t=0\}. 
\end{aligned}
\end{equation*}
Note that 
\[
\epslamN = \partial_\nu \UN|_{(0,T) \times \partial \Omega}. 
\]

We integrate by parts to have 
\begin{align*}
   &\inttp \epslamN f_0 \diff S \diff t = \inttp \partial_\nu \UN f_0 \diff S \diff t\\
 = &\inttx \Delta \UN u_0 \dxt + \inttx \nabla \UN \cdot \nabla u_0 \dxt\\
 = &\inttx \Delta \UN u_0 \dxt - \inttx \UN \cdot \Delta u_0 \dxt\\
 = &\inttx \frac{1}{c^2(x)} \partial_t^2 \UN u_0 - B_N(\beta_1, \ldots, \beta_{N-1}; u_1, \ldots, u_N) u_0 \dxt - \inttx \UN  \Delta u_0 \dxt\\
 = &\inttx \UN \frac{1}{c^2(x)} \partial_t^2 u_0  - B_N(\beta_1, \ldots, \beta_{N-1}; u_1, \ldots, u_N) u_0 \dxt - \inttx \UN  \Delta u_0 \dxt\\
 = &\inttx \UN (\frac{1}{c^2(x)} \partial_t^2 - u_0 \Delta u_0 ) \dxt- \inttx B_N(\beta_1, \ldots, \beta_{N-1}; u_1, \ldots, u_N) u_0 \dxt \\
 = &- \inttx R_N(\beta_1, \ldots, \beta_{N-2}; u_1, \ldots, u_N) u_0 \dxt  - \inttx N! \beta_{N-1}(x) \partial_t^2 (u_1u_2 \ldots u_N)  u_0 \dxt\\
 = &- \inttx R_N(\beta_1, \ldots, \beta_{N-2}; u_1, \ldots, u_N) u_0 \dxt  + \inttx N! \beta_{N-1}(x) \partial_t (u_1u_2 \ldots u_N)  \partial_t u_0 \dxt. \\
\end{align*}
We are going to use a inductive procedure to determine the nonlinear coefficients. 
Specially, assuming we have determined $\beta_1, \ldots, \beta_{N-2}$, we consider the determination of $\beta_{N_1}$. 
It follows that the first term is known and we need to determine $\beta_{N_1}$ from 
\[
I_{N-1} = \inttx N! \beta_{N-1}(x) \partial_t (u_1u_2 \ldots u_N)  \partial_t u_0 \dxt. 
\]

==> recoveryN.tex <==
\section{Recovery for higher order terms}\label{sec_hN}
%We have the following corollary by Lemma \ref{lm_fourwaves}.
In this subsection we use Lemma \ref{lm_psmodel} 
{\color{Blue} (or Lemma \ref{lm_psmodel_v})}
to analyze each term in (\ref{eq_h1}), (\ref{eq_h2}), as well as (\ref{eq_h3}) and we apply $Q_g$ to them by Lemma \ref{lm_psmodel2} {\color{Blue} (or Lemma \ref{lm_psmodel2_v})}. 
{\color{Blue}Note that we use the blue color to denote the arguments using Piriou conformal distributions. 
For this part, we always assume $v_1 \in \Ir^\mu(M;K)$ according to Lemma \ref{lm_v1}. 
}

For convenience, we assume $A_N \neq 0$, $h_N \neq 0$ for the moment. 
\subsubsection{The analysis of (\ref{eq_h1})}
Recall in (\ref{eq_h1}) we have
\begin{align*}
\partial^{2N-2}_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} (H_1 )|_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0} 
=    \iota  \sum_{(j, k,l) = \Sigma(\{2, 3, 4\})}
%\lge A_N, \diff \big(
%\cjv_1^{N} v_1^{N - 2} v_j v_k v_l
%+ 3 \cjv_1^{N-1} v_1^{N-1} v_j v_k  \cjv_l + \nonumber\\
%& \quad \quad \quad  \quad \quad \quad \quad \quad \quad \quad \quad \quad 
%+ 3\cjv_1^{N-2} v_1^{N} v_j \cjv_k  \cjv_l 
%+\cjv_1^{N-3} v_1^{N+1} \cjv_j \cjv_k \cjv_l
%\big) 
%\rge_g.
\lge A_N, \diff \big(W_1 + W_2 + W_3 +W_4\big) 
\rge_g,
\end{align*}
where 
\begin{align*}
&W_1 \coloneqq C_3\cjv_1^{N} v_1^{N - 2} v_j v_k v_l, 
&W_2 \coloneqq C_2 \cjv_1^{N-1} v_1^{N-1} v_j v_k  \cjv_l, \\
&W_3 \coloneqq C_1\cjv_1^{N-2} v_1^{N} v_j \cjv_k  \cjv_l, 
&W_4 \coloneqq C_0 \cjv_1^{N-3} v_1^{N+1} \cjv_j \cjv_k \cjv_l. 
\end{align*}
Take the last term $ W_4$ %$\lge A_N, \diff (\cjv_1^{N-3} v_1^{N+1} \cjv_j \cjv_k \cjv_l)\rge_g$ 
for example. 
We plug $w_1 = v_1$ and $w_j = \cjv_j$ for $j=2,3,4$ into Lemma \ref{lm_psmodel}.  
Then microlocally away from $\Xi_4$, we have
\begin{align*}
W_4 %\coloneqq \cjv_1^{N-3} v_1^{N+1} \cjv_j \cjv_k \cjv_l 
\in \sum_{l=1}^{2N-2} \Icl^{4\mu+3+ (l-1)(\mu + \frac{3}{2})}(\Lambda_q)
\end{align*}
with the homogeneous term of degree $\mu(2N-2,4)$ given by 
\begin{align*}
&\sigma_{\mu(2N-2,4)}(W_4)(q, \zeta) 
= C_0(2\pi)^{-3} \sigma_{\mu(2N-2,1)}(v_1^{N-3}(\cjv_1)^{N+1})(q, \zeta^{(1)})
\prod_{m=j,k,l} \overline{{\sigmp}(v_m)(q, -\zeta^{(m)})}.
%&  \quad \times \underbrace{{\sigmp}(v_1) \ast \ldots \ast {\sigmp}(v_1) }_{\alpha} \ast
%\underbrace{{\sigmp}(\cjv_1) \ast \ldots \ast {\sigmp}(\cjv_1) }_{\beta}(q, \zeta^{(1)})
%\prod_{j=2}^{4} {\sigmp}(v_j)(q, \zj), \nonumber
\end{align*}
{\color{Blue}
Alternatively, by Lemma \ref{lm_psmodel_v}, microlocally away from $\Xi_4$, we obtain
\begin{align*}
W_4 %\coloneqq \cjv_1^{N-3} v_1^{N+1} \cjv_j \cjv_k \cjv_l 
\in  \Ical^{4\mu+3+ (2N-3)(\mu + \frac{3}{2})}(\Lambda_q)
\end{align*}
with the principal symbol given by 
\begin{align*}
&{\sigmp}(W_1)(q, \zeta) 
= C_0(2\pi)^{-3} {\sigmp}(v_1^{N-3}(\cjv_1)^{N+1})(q, \zeta^{(1)})
\prod_{m=j,k,l} \overline{{\sigmp}(v_m)(q, -\zeta^{(m)})}.
%&  \quad \times \underbrace{{\sigmp}(v_1) \ast \ldots \ast {\sigmp}(v_1) }_{\alpha} \ast
%\underbrace{{\sigmp}(\cjv_1) \ast \ldots \ast {\sigmp}(\cjv_1) }_{\beta}(q, \zeta^{(1)})
%\prod_{j=2}^{4} {\sigmp}(v_j)(q, \zj), \nonumber
\end{align*}
}
\begin{remark}\label{rm_N3N2}
Note we would like to choose special $v_j$ such that only a few terms have nonvanishing homogeneous term of degree $\mu(2N-2, 4)$. ({\color{Blue}Alternatively, only a few terms have nonvanishing principal symbol.})
Note we have two different cases, $N=2$ and $N \geq 3$, see Remark \ref{rm_N2}.
Since they have different terms, we cannot analyze them at the same time so we would like to use different schemes for them.
When $N =2$, this can be achieved by choosing $f_2, f_3, f_4$ as in Remark \ref{rm_fj}, such that 
\[{\sigmp}(v_j) \neq  0 \text{ near } (q, \zj), \quad 
{\sigmp}(v_j) = 0 \text{ near } (q, -\zj), \quad j = 2,3,4.
\] 
When $N \geq 3$, we choose $f_2, f_3, f_4$ such that 
\[{\sigmp}(v_j) =  0 \text{ near } (q, \zj), \quad 
{\sigmp}(v_j)\neq 0 \text{ near } (q, -\zj), \quad j = 2,3,4.
\] 
\end{remark}
In the following, we consider $N \geq 3$ first. 
One can follow the similar arguments to analyze the case $N=2$. 

With the remark above, we have $W_2, W_3, W_4 $ away from $\Xi_4$ are in the same polyhomogeneous conormal distribution class as $W_1$ but with
\[
\sigma_{\mu(2N-2,4)}(W_1)(q, \zeta)  = \sigma_{\mu(2N-2,4)}(W_2)(q, \zeta)  = \sigma_{\mu(2N-2,4)}(W_3)(q, \zeta)  = 0. 
\]
{\color{Blue}
Alternatively, in this case, we have $W_2, W_3, W_4 $ away from $\Xi_4$ are in 
$\Ical^{4\mu+3+ (2N-3)(\mu + \frac{3}{2})}(\Lambda_q)$ but with
    \[
    {\sigmp}(W_1)(q, \zeta)  = {\sigmp}(W_2)(q, \zeta)  = {\sigmp}(W_3)(q, \zeta)  = 0. 
    \]}

Additionally, we pick $v_1$ as a real distribution such that Remark \ref{rm_v1pick} holds. 
Then by Lemma \ref{lm_pld}, we have
\begin{align*}
\lge A_N, \diff \big(W_1 + W_2 + W_3 +W_4\big) \rge_g 
\in \sum_{l=1}^{2N-2} \Icl^{4\mu+4 + (l-1)(\mu + \frac{3}{2})}(\Lambda_q)
\end{align*}
with 
\begin{align*}
&\sigma_{\mu(2N-2,4)+1}(\lge A_N, \diff \big(W_1 + W_2 + W_3 +W_4\big) \rge_g )(q, \zeta) \\
= &\iota  C_0(2\pi)^{-3} \lge A_N, \zeta \rge_g
\sigma_{\mu(2N-2,1)}(v_1^{N-3}(\cjv_1)^{N+1})(q, \zeta^{(1)}) 
\prod_{m=j,k,l} \overline{{\sigmp}(v_m)(q, -\zeta^{(m)})}\\
= & \iota C_0 (2\pi)^{-3} \lge A_N, \zeta \rge_g
\sigma_{\mu(2N-2,1)}(v_1^{2N-2}) (q, \zeta^{(1)}) 
\prod_{m=j,k,l} \overline{{\sigmp}(v_m)(q, -\zeta^{(m)})}.
\end{align*}
The last equality comes from Remark \ref{rm_v1pick}. 
{\color{Blue} Alternatively, we have
    \begin{align*}
    \lge A_N, \diff \big(W_1 + W_2 + W_3 +W_4\big) \rge_g 
    \in  \Ical^{4\mu+4 + (2N-3)(\mu + \frac{3}{2})}(\Lambda_q)
    \end{align*}
    with 
    \begin{align*}
    &{\sigmp}(\lge A_N, \diff \big(W_1 + W_2 + W_3 +W_4\big) \rge_g )(q, \zeta) \\
    = &\iota  C_0(2\pi)^{-3} \lge A_N, \zeta \rge_g
    {\sigmp}(v_1^{N-3}(\cjv_1)^{N+1}) (q, \zeta^{(1)}) 
    \prod_{m=j,k,l} \overline{{\sigmp}(v_m)(q, -\zeta^{(m)})}\\
    = & \iota C_0(2\pi)^{-3} \lge A_N, \zeta \rge_g
    {\sigmp}(v_1^{2N-2}) (q, \zeta^{(1)}) 
    \prod_{m=j,k,l} \overline{{\sigmp}(v_m)(q, -\zeta^{(m)})}.
    \end{align*}
    As we can see, the only difference for these two methods is that we replace the class of polyhomogeneous conormal distributions \[\sum_{l=1}^{2N-2} \Icl^{4\mu+4 + (l-1)(\mu + \frac{3}{2})}(\Lambda_q)\]
    by a class of conormal distributions $\Ical^{4\mu+4 + (2N-3)(\mu + \frac{3}{2})}(\Lambda_q)$ with $l=2N-2$. Also, the homogeneous term in the full symbol will be replaced by the principal symbol. 
    Thus, we omit these difference in the following and only state the different results for Proposition
    \ref{pp_uNN}. 
}

Then by Lemma \ref{lm_psmodel}, away from $\Xi_4$ we have 
\[
\partial^{2N-2}_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} (H_1 )|_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0} \in \sum_{l=1}^{2N-2} \Icl^{(l+3)\mu + l + 3}(\Lambda_q).
\]
The homogeneous term $\sigma_{\mu(2N-2,4)}(\partial^{2N-2}_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} (H_1 )|_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0})$ can be directly derived from the computation above.  
Finally, we conclude by Lemma \ref{lm_Qgcl} or Lemma \ref{lm_psmodel2} that away from $\unionGammas$ one has
\begin{align*}
\partial^{2N-2}_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} (Q_g(H_1) )|_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0} \in \sum_{l=1}^{2N-2} \Icl^{4\mu + (l-1)(\mu + \frac{3}{2}) + \frac{5}{2}}(\Lambda_q^g \setminus \Lambda_q). 
\end{align*}
%Let $(y, \eta)$ be a lightlike covector lying along a forward null bicharacteristic of $\square_g$ starting from $(q, \zeta) \in \Lambda_q$. 
%We assume $(y, \eta)$ % \in \nxxi$ and 
%is away from $\unionGammas$. 
%Then 
%\begin{align*}
%\mathcal{S}(y, \eta, q, \zeta) = {\sigmp}(Q_g)(y, \eta,q, \zeta) \sigma_{\mu(2N-2,1)}(v_1^{2N-2}) (q,  \zeta^{(1)})
%\prod_{j=2}^{4} {\sigmp}(\cjv_j)(q, -\zj).
%\end{align*}
If $(y, \eta) \in \Tq$ with $(q, \zeta) \in \Lambda_q$
is away from $\unionGammas$,
then 
the homogeneous term of degree $\mu(2N+1,4)+1-3/2 = \mu(2N+1,4)-1/2$ in its full symbol is given by 
\begin{align}\label{eq_H1ps}
&\sigma_{\mu(2N+1,4)- 1/2}(\partial^{2N-2}_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} (Q_g(H_1) )|_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0})(y,\eta)\\
=& 
\begin{multlined}[t][0.9\linewidth]
- 6C_0(2\pi)^{-2N}  
{\sigmp}(Q_g)(y, \eta,q, \zeta) \times \\
\times \lge A_N, \zeta \rge_g \sigma_{\mu(2N-2, 1)}(v_1^{2N-2}) (q, \zeta^{(1)}) 
\prod_{j=2}^{4} \overline{{\sigmp}(v_j)(q, -\zj)}. 
\end{multlined}
\nonumber
\end{align}

\subsubsection{The analysis of (\ref{eq_h2})}
Next, we analyze (\ref{eq_h2}) in a similar way. By choosing $v_1, v_2, v_3, v_4$ with special principal symbols, we observe that the only term in (\ref{eq_h2}) with nonvanishing desired homogeneous term is the last one
\[
W_5 \coloneqq E_0\lge A_N, \diff v_1 \rge_g (\cjv_1^{N-3} v_1^{N} \cjv_j \cjv_k \cjv_l). 
\]
Note this time by Lemma \ref{lm_pld} we have 
\[
\lge A_N, \diff v_1 \rge_g \in I^{\mu+1}(\Lambda_1), \text{ with } {\sigmp}(\lge A_N, \diff v_j \rge_g)(q, \zeta^{(1)}) = \iota \lge A_N, \zeta^{(1)} \rge_g {\sigmp}(v_1)(q, \zeta^{(1)}). 
\]
We compute $\lge A_N, \diff v_1 \rge_g \cjv_1^{N-3} v_1^{N}$ by Claim \ref{cl_conv} to have
\begin{align*}
\lge A_N, \diff v_1 \rge_g \cjv_1^{N-3} v_1^{N} 
\in \sum_{l=1}^{2N-2} \Icl^{\mu + 1 + (l-1)(\mu + \frac{3}{2})}(\Lambda_1),
\end{align*}
and the desired homogeneous term is 
\begin{align*}
&\sigma_{\mu(2N-2,1)+1}(\lge A_N, \diff v_1 \rge_g \cjv_1^{N-3} v_1^{N} ) \\
=& \iota (2\pi)^{-(2N-3)}( \lge A_N, \ \cdot \ \rge_g {\sigmp}(v_1))\ast 
\underbrace{{\sigmp}(v_1) \ast \ldots \ast {\sigmp}(v_1) }_{N} \ast
\underbrace{{\sigmp}(\cjv_1) \ast \ldots \ast {\sigmp}(\cjv_1) }_{N-3}.
\end{align*}
Applying Remark \ref{rm_v1pick},  at $(q, \zeta^{(1)})\in \Lambda_1$ one has
\begin{align*}
&\sigma_{\mu(2N-2,1)+1}(\lge A_N, \diff v_1 \rge_g \cjv_1^{N-3} v_1^{N} ) 
%=& \iota (2\pi)^{-(2N-3)}( \lge A_N, \ \cdot \ \rge_g {\sigmp}(v_1))\ast 
%\underbrace{{\sigmp}(v_1) \ast \ldots \ast {\sigmp}(v_1) }_{2N-3} \\
=  \sigma_{\mu(2N-2,1)+1}(\lge A_N, \diff v_1 \rge_g v_1^{2N-3} ) \\
= & \frac{1}{2N-2}\sigma_{\mu(2N-2,1)+1}(\lge A_N, \diff v_1^{2N-2} \rge_g )
= \frac{1}{2N-2}\lge A_N, \zeta^{(1)} \rge_g \sigma_{\mu(2N-2,1)+1}( v_1^{2N-2} ). 
\end{align*}
Thus, we apply Lemma \ref{lm_psmodel} and Lemma \ref{lm_Qgcl} to have the following description for the second part. 
Away from $\unionGammas$, one has
\begin{align*}
\partial^{2N-2}_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} (Q_g(H_2) )|_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0} \in \sum_{l=1}^{2N-2} \Icl^{4\mu+ (l-1)(\mu + \frac{3}{2}) + \frac{5}{2}}(\Lambda_q^g \setminus \Lambda_q). 
\end{align*}
%Let $(y, \eta)$ be a lightlike covector lying along a forward null bicharacteristic of $\square_g$ starting from $(q, \zeta) \in \Lambda_q$. 
%We assume $(y, \eta)$ % \in \nxxi$ and 
%is away from $\unionGammas$. 
%Then 
If $(y, \eta) \in \Tq$ with $(q, \zeta) \in \Lambda_q$
is away from $\unionGammas$,
then 
the homogeneous term of degree $\mu(2N-2,4)+1 -3/2 = \mu(2N-2,4)-1/2$ in its full symbol is given by 
\begin{align}\label{eq_H2ps}
&\sigma_{\mu(2N-2,4)-1/2}(\partial^{2N-2}_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} (Q_g(H_2) )|_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0}) (y, \eta) = \\
%= &  -6(2\pi)^{-2N} 
%{\sigmp}(Q_g)(y, \eta,q, \zeta)\lge A_N, \zeta \rge_g \sigma_{(2N-2)\mu + (2N-3)}(v_1^{N-3}(\cjv_1)^{N+1}) 
%\prod_{j=2}^{4} {\sigmp}(\cjv_j)(q, -\zj) \nonumber \\
= & 
\begin{multlined}[t][0.9\linewidth]
- \frac{6E_0}{2N-2}(2\pi)^{-2N} {\sigmp}(Q_g)(y, \eta,q, \zeta) \times \\
\times \lge A_N, \zeta^{(1)} \rge_g \sigma_{\mu(2N-2,1)}(v_1^{2N-2}) 
\prod_{j=2}^{4} {\sigmp}(\cjv_j)(q, -\zj). 
\end{multlined}
\nonumber
\end{align}

\subsubsection{The analysis of (\ref{eq_h3})} Third, we consider each term in (\ref{eq_h3}). 
This time a direct application of Lemma \ref{lm_psmodel} and Lemma \ref{lm_psmodel2} imply that
\[
\partial^{2N-2}_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} (Q_g(H_3) )|_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0} \in \sum_{l=1}^{2N-2} \Icl^{4\mu + (l-1)(\mu + \frac{3}{2}) + \frac{3}{2}}(\Lambda_q^g \setminus \Lambda_q). 
\]
%Let $(y, \eta)$ be a lightlike covector lying along a forward null bicharacteristic of $\square_g$ starting from $(q, \zeta) \in \Lambda_q$. 
%We assume $(y, \eta)$ % \in \nxxi$ and 
%is away from $\unionGammas$. 
%Then 
If $(y, \eta) \in \Tq$ with $(q, \zeta) \in \Lambda_q$
is away from $\unionGammas$,
then 
the homogeneous term of degree $\mu(2N-2,4)-3/2$ in its full symbol is given by 
\begin{align}\label{eq_H3ps}
&\sigma_{\mu(2N-2,4)-3/2}(\partial^{2N-2}_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} (Q_g(H_3) )|_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0}) (y, \eta)\\
= & 6 F_0{\sigmp}(Q_g)(y, \eta,q, \zeta)  
%= &  -6(2\pi)^{-2N} 
%{\sigmp}(Q_g)(y, \eta,q, \zeta)\lge A_N, \zeta \rge_g \sigma_{(2N-2)\mu + (2N-3)}(v_1^{N-3}(\cjv_1)^{N+1}) 
%\prod_{j=2}^{4} {\sigmp}(\cjv_j)(q, -\zj) \nonumber \\
\begin{multlined}[t][0.7\linewidth]
 (  \iota \divg(A_N) + \sum_{\alpha+ \beta=N}\lge  A_\alpha, A_\beta \rge_g + h_{N}) \times{}  \\
\times \sigma_{\mu(2N-2,1)}(v_1^{2N-2}) (q, \zeta^{(1)})
\prod_{j=2}^{4} \overline{{\sigmp}(v_j)(q, -\zj)}.
\end{multlined}\nonumber
\end{align}

\subsubsection{The analysis of $\mathcal{U}^{2N+1}_{N}$}
We summarize the analysis of (\ref{eq_h1})-(\ref{eq_h3}) and describe the singularities of (\ref{eq_uNN}) in the following proposition. 
%{\color{Brown} For simplification, currently we assume $A_N \neq 0$ for all $N \geq 1$. }
%%%%%%%%%%%%%%%%%%%% remark %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%First we choose special $f_1, f_2, f_3, f_4$ by Remark \ref{rm_v1pick} and Remark \ref{rm_N3N2} such that most terms will vanish. 
%\begin{remark}\label{rm_f4}
%    %Note that 
%    %We choose special $v_j$ such that most terms will vanish.
%    %This can be achieved by choosing $f_1, \ldots, f_4$ by Remark \ref{rm_v1pick} and Remark \ref{rm_fj}, such that
%    Given $(q, \zj) \in N^*K_j$, we can choose  $f_1, \ldots, f_4$ such that
%    \begin{itemize}
%        \item[(1)] ${\sigmp}(v_1)(x, \xi)  = \overline{{\sigmp}(v)(x, -\xi)}$ near  $(q, \zeta^{(1)})$ with $\sigma_{\mu(2N-2,1)}(v_1^{2N-2}) (q,  \zeta^{(1)}) \neq 0$,
%        \item[(2)] ${\sigmp}(v_j) =  0$ near $(q, \zj)$ and
%        $ {\sigmp}(v_j)\neq 0$ near $(q, -\zj)$, for $j = 2,3,4$.
%        %\item[(2)] 
%    \end{itemize}
%    %We emphasize that 
%\end{remark}
%%%%%%%%%%%%%

\begin{pp}\label{pp_uNN}
    %Suppose $\gamma_{x_j, \xi_j}(t), \ j = 1,2,3$ intersect regularly at $q$. 
    Assume $K_1, K_2, K_3, K_4$ intersect 4-transversally at $q$, see Definition \ref{df_intersect}. %(order???)
    Let $\mu <-\frac{3}{2}$ be an irrational real number. 
    Recall the decomposition in (\ref{eq_uNNde}) with  $N \geq 2$. 
    Let $f_1, \ldots, f_4$ be chosen in  Remark \ref{rm_v1pick} and \ref{rm_N3N2}. 
    Assume $A_N \neq 0$ at $q$. 
    %Let $\Lambda_q^g$ be the flow out of $\Lambda_q$ under the Hamilton flow of $\square_g$. 
    Then %in $\nxxi$ and 
    away from $\unionGammas$, one has 
    \[
    \mathcal{U}^{2N+1}_{N, 0} \in \sum_{l=1}^{2N-2} \Icl^{4\mu + (l-1)(\mu + \frac{3}{2}) +  \frac{5}{2}}(\Lambda_q^g \setminus \Lambda_q), \quad  
    \mathcal{U}^{2N+1}_{N, 1} \in \sum_{l=1}^{2N-2} \Icl^{4\mu+ (l-1)(\mu + \frac{3}{2}) +\frac{3}{2} }(\Lambda_q^g \setminus \Lambda_q). 
    \]
    Moreover, 
    %let $(y, \eta)$ be a lightlike covector lying along a forward null bicharacteristic of $\square_g$ starting from $(q, \zeta) \in \Lambda_q$. 
    %Assume $(y, \eta)$ % \in \nxxi$ and 
    %is away from $\unionGammas$. 
    if $(y, \eta) \in \Tq$ with $(q, \zeta) \in \Lambda_q$
    is away from $\unionGammas$ (see (\ref{def_Gammas0})),
    then 
    for $N \geq 3$ we have %the principal symbol of $\mathcal{U}^{(3)}$ at $(y, \eta)$ is given by 
    \begin{align}
    &\sigma_{\mu(2N-2,4)- 1/2}(\mathcal{U}^{2N+1}_{N, 0} ) (y,\eta) 
    = - c_N
     \big(\lge A_N, \zeta 
    +\frac{1}{2N-2}  \zeta^{(1)} \rge_g \big)\mathcal{S}, %(y, \eta, q, \zeta),
    \label{ps_uNN0}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &\sigma_{\mu(2N-2,4)- 3/2}(\mathcal{U}^{2N+1}_{N, 1} ) (y, \eta) 
    = c_N
    (  \iota \divg(A_N) + \sum_{\alpha+ \beta=N}\lge  A_\alpha, A_\beta \rge_g + h_{N}) 
    \mathcal{S}, \label{ps_uNN1}
    \end{align}
%    \begin{align*}
%    &\sigma_{\mu(2N+1,4)- 1/2}(\mathcal{U}^{2N+1}_{N, 0} ) 
%    = - 6 (2\pi)^{-2N} {\sigmp}(Q_g)(y, \eta,q, \zeta) \\ 
%    &\times \big( \lge A_N, \zeta \rge_g
%    +\frac{1}{2N-2}   \lge A_N, \zeta^{(1)} \rge_g \big)
%     \sigma_{\mu(2N-2,1)}(v_1^{2N-2}) (q,  \zeta^{(1)})
%    \prod_{j=2}^{4} {\sigmp}(\cjv_j)(q, -\zj). 
%    \nonumber\\
%    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    &\sigma_{\mu(2N+1,4)- 3/2}(\mathcal{U}^{2N+1}_{N, 1} ) 
%    =  6 (2\pi)^{-2N} {\sigmp}(Q_g)(y, \eta,q, \zeta)  
%    (  \iota \divg(A_N) + \sum_{\alpha+ \beta=N}\lge  A_\alpha, A_\beta \rge_g + h_{N}) \nonumber \\
%    &\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad   \times \sigma_{\mu(2N-2,1)}(v_1^{2N-2}) 
%    \prod_{j=2}^{4} {\sigmp}(\cjv_j)(q, -\zj),
%    \nonumber
%    \end{align*}
    where $c_N =  6^2 {N \choose 3}(2\pi)^{-2N} $, the decomposition $\zeta = \sum_{j=1}^4\zj$ with $\zj \in \Lambda_j$ is unique, and $\mathcal{S}$ denotes
    \begin{align*}
    \mathcal{S}(y, \eta, q, \zeta) = {\sigmp}(Q_g)(y, \eta,q, \zeta) \sigma_{\mu(2N-2,1)}(v_1^{2N-2}) (q,  \zeta^{(1)})
    \prod_{j=2}^{4} {\sigmp}(\cjv_j)(q, -\zj).
    \end{align*}
    If $A_N = 0$ near $q$ and $h_N(q) \neq 0$, then 
    \[
    \mathcal{U}^{2N+1}_{N} = \mathcal{U}^{2N+1}_{N, 1} \in \sum_{l=1}^{2N-2} \Icl^{4\mu+ (l-1)(\mu + \frac{3}{2}) +\frac{3}{2} }(\Lambda_q^g \setminus \Lambda_q),
    \]
    with principal symbol given by (\ref{ps_uNN1}).
    %\begin{align*}
    %\mathcal{A}_{3,0}(\zeta^{(1)}, \zeta^{(2)}, \zeta^{(3)})
    %= 
    %\sum_{(i,j,k) \in  \Sigma(3)}
    %\lge A_1, \zeta^{(i)} + 3\zeta^{(j)} \rge_g \overline{\sigma_i(z, -\zeta^{(i)})} \sigma_j(z, \zeta^{(j)})\sigma_k(z, \zeta^{(k)}). 
    %\end{align*}
    When $N=2$, we have a similar description with
     \begin{align}
    &\sigma_{\mu(2,4)- 1/2}(\mathcal{U}^{5}_{2, 0} ) (y,\eta) 
    = -  6(2\pi)^{-4} 
    \big( \lge A_2, 8\zeta -2 \zeta^{(1)} \rge_g \big)\mathcal{S}(y, \eta, q, \zeta),\label{ps_uNN0_N2} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &\sigma_{\mu(2,4)- 3/2}(\mathcal{U}^{5}_{2, 1} ) (y, \eta) 
     =  6 (2\pi)^{-4} 
    (  \iota \divg(A_2) + \lge  A_1, A_1 \rge_g + h_{2}) 
    \mathcal{S}(y, \eta, q, \zeta). \label{ps_uNN1_N2}
    \end{align}
\end{pp}
{\color{Blue} \noindent
    Alternatively, we have the following proposition for $\mathcal{U}^{2N+1}_{N}$ using Piriou conormal distributions.
\begin{pp}\label{pp_uNN_v}
    %Suppose $\gamma_{x_j, \xi_j}(t), \ j = 1,2,3$ intersect regularly at $q$. 
    Assume $K_1, K_2, K_3, K_4$ intersect 4-transversally at $q$, see Definition \ref{df_intersect}. %(order???)
    Let $\mu <-\frac{3}{2}$ such that $\mu + \frac{1}{2} \notin \mathbb{Z}$. 
    Recall the decomposition in (\ref{eq_uNNde}) with  $N \geq 2$. 
    Let $f_1, \ldots, f_4$ be chosen in Remark \ref{rm_v1pick} and \ref{rm_N3N2}.
    In particular, we assume $v_1 \in \Ir^\mu(M;K_1)$ by subtracting a smooth error.
    Assume $A_N \neq 0$ at $q$. 
    %Let $\Lambda_q^g$ be the flow out of $\Lambda_q$ under the Hamilton flow of $\square_g$. 
    Then %in $\nxxi$ and 
    away from $\unionGammas$, one has 
    \[
    \mathcal{U}^{2N+1}_{N, 0} \in  \Ical^{4\mu + (2N-3)(\mu + \frac{3}{2}) +  \frac{5}{2}}(\Lambda_q^g \setminus \Lambda_q), \quad  
    \mathcal{U}^{2N+1}_{N, 1} \in \Ical^{4\mu+ (2N-3)(\mu + \frac{3}{2}) +\frac{3}{2} }(\Lambda_q^g \setminus \Lambda_q). 
    \]
    Moreover, 
    if $(y, \eta) \in \Tq$ with $(q, \zeta) \in \Lambda_q$
    is away from $\unionGammas$ (see (\ref{def_Gammas0})),
    then for $N \geq 3$ we have
    %let $(y, \eta)$ be a lightlike covector lying along a forward null bicharacteristic of $\square_g$ starting from $(q, \zeta) \in \Lambda_q$. 
    %Assume $(y, \eta)$ % \in \nxxi$ and 
    %is away from $\unionGammas$. 
    %Then we have %the principal symbol of $\mathcal{U}^{(3)}$ at $(y, \eta)$ is given by 
    \begin{align}
    &{\sigmp}(\mathcal{U}^{2N+1}_{N, 0} ) (y,\eta) 
    = - c_N 
    \big( \lge A_N, \zeta +
    \frac{1}{2N-2}  \zeta^{(1)} \rge_g \big)\mathcal{S}, %(y, \eta, q, \zeta),\nonumber \\
    \label{ps_uNN0_v}\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &{\sigmp}(\mathcal{U}^{2N+1}_{N, 1} ) (y, \eta) 
    =  c_N
    (  \iota \divg(A_N) + \sum_{\alpha+ \beta=N}\lge  A_\alpha, A_\beta \rge_g + h_{N}) 
    \mathcal{S}, \label{ps_uNN1_v}
    \end{align}
    where $c_N =  6^2 {N \choose 3}(2\pi)^{-2N} $, the decomposition $\zeta = \sum_{j=1}^4\zj$ with $\zj \in \Lambda_j$ is unique, and $\mathcal{S}$ denotes
    \begin{align*}
    \mathcal{S}(y, \eta, q, \zeta) = {\sigmp}(Q_g)(y, \eta,q, \zeta) {\sigmp}(v_1^{2N-2}) (q,  \zeta^{(1)})
    \prod_{j=2}^{4} {\sigmp}(\cjv_j)(q, -\zj).
    \end{align*}
    If $A_N = 0$ near $q$ and $h_N(q) \neq 0$, then 
    \[
    \mathcal{U}^{2N+1}_{N} = \mathcal{U}^{2N+1}_{N, 1} \in \Ical^{4\mu+ (2N-3)(\mu + \frac{3}{2}) +\frac{3}{2} }(\Lambda_q^g \setminus \Lambda_q),
    \]
    with principal symbol given by (\ref{ps_uNN1_v}).
    When $N=2$, we have a similar description with
    \begin{align}
    &{\sigmp}(\mathcal{U}^{5}_{2, 0} ) (y,\eta) 
    = -  6(2\pi)^{-4} 
    \big( \lge A_2, 8\zeta -2 \zeta^{(1)} \rge_g \big)\mathcal{S}(y, \eta, q, \zeta),\label{ps_uNN0_v_N2} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &{\sigmp}(\mathcal{U}^{5}_{2, 1} ) (y, \eta) 
    =  6 (2\pi)^{-4} 
    (  \iota \divg(A_2) + \lge  A_1, A_1 \rge_g + h_{2}) 
    \mathcal{S}(y, \eta, q, \zeta). \label{ps_uNN1_v_N2}
    \end{align}
\end{pp}
}
\subsection{Recovery of $A_N$ and $h_N$ for $N \geq 2$}
%For $k =1, 2$, let $u^{(j)}$ solve the semilinear wave equation (\ref{eq_source-problem}) with $A^{(k)}(x, u)$ and $h^{(k)}(x,u)$ satisfying (\ref{assump_Ah}). 
%Suppose the source-to-solution map 
%\[
%L^{(1)}_{A^{(1)}, h^{(1)}}(f) = L^{(2)}_{A^{(2)}, h^{(2)}}(f) 
%\]
%for small data $f$ with $\supp(f) \subset V$.
 
In this subsection, we determine $A_N$ and $h_N$ from the $(2N+1)$th linearization of the source to solution map, assuming that
\[
L_{A^{(1)}, h^{(1)}}(f) = L_{A^{(2)}, h^{(2)}}(f),
\]
and for $j < N$ we have %we have recovered $A_j, h_j$ for $j < N$, i.e.
\[
A_j^{(1)} = A_j^{(2)}, \quad h_j^{(1)} = h_j^{(2)}.
\]
We note that this is true for $N=1$ by Section \ref{subsec_planewaves}. 

For any $q \in I(p^-, p^+)$, by \cite[Lemma 3.5]{Kurylev2018}, 
we can find lightlike vectors $(x_j, \xi_j)_{j=1}^4$ 
such that they are causally independent
as in (\ref{assump_xj}) and the four null geodesics corresponding to $(x_j, \xi_j)$ intersect regularly at $q$.  
Then we construct $K_j, \Sigma_j, \Lambda_j$ for such $(x_j, \xi_j)$ with sufficiently small $s_0$, so that $K_1, K_2, K_3, K_4$ intersect 4-transversally at $q$. 
%Suppose $q = \gamma_{x_j, \xi_j}(t_j)$.  

By Lemma \ref{lm_3null}, there exist $\zeta \in L_q^{*,+} M$ and $(y, \eta) \in L^{*,+}V$ 
satisfying 
$(y,\eta) = \mathcal{C}^{\text{reg}}(q, \zeta, t_y)$.
Note that %$\dot{\gamma}_{x_j, \xi_j}(t_j)$ are linearly independent so 
$\zeta$ has a unique decomposition $\zeta = \sum_{j=1}^4 \zj$ with $\zj \in \Lambda_j$. %, for $j = 1,2,3,4$. 
Then according to Remark \ref{rm_v1pick} and \ref{rm_N3N2}, we choose special $f_1, \ldots, f_4$ and set $f = \sum_{j=1}^4 \ep_j f_j$.
Recall in (\ref{eq_LfN}) we consider the $(2N+1)$th linearization  
\begin{align*}
\mathcal{U}^{2N+1,k} %= \partial_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3} L_{A,h}(f) |_{\epsilon_1 = \epsilon_2 = \epsilon_3=0}
= \partial^{2N-2}_{\epsilon_1}\partial_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} L_{A^{(k)}, h^{(k)}}(f) |_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0}, \quad k = 1,2.
\end{align*}
In (\ref{eq_uNNN}), we obtain that %$L_{A^{(1)}, h^{(1)}}(f) = L_{A^{(2)}, h^{(2)}}(f)$ implies
$\mathcal{U}^{2N+1,1}_N = \mathcal{U}^{2N+1,2}_N$. 
Now we can use Proposition \ref{pp_uNN} to get information from the leading singularities at $(y, \eta) \in L^*V$, for $(y, \eta)$ in the forward bicharacteristic from $(q, \zeta)$ and away from $\unionGammas$. 
Indeed, when $N=2$, 
we compare the homogeneous term of order $(\mu(2,4)- 1/2)$
in (\ref{ps_uNN0_N2}) ({\color{Blue}or the principal symbol in (\ref{ps_uNN0_v_N2})}) at $(y, \eta)$ for $k=1,2$ to have
\begin{align*}
&\lge A_2^{(1)}, 8\zeta 
- 2\zeta^{(1)} \rge_g  = \lge A_2^{(2)}, 8\zeta 
- 2\zeta^{(1)} \rge_g.
\end{align*}
When $N \geq 3$, 
we compare the homogeneous term of order $\mu(2N-2,4)- 1/2$ in (\ref{ps_uNN0}) ({\color{Blue}or the principal symbol in (\ref{ps_uNN0_v})}) at $(y, \eta)$ for $k=1,2$ to have
\begin{align*}
&\lge A_N^{(1)}, \zeta 
+\frac{1}{2N-2}   \zeta^{(1)} \rge_g  = 
\lge A_N^{(2)}, \zeta 
+\frac{1}{2N-2}  \zeta^{(1)} \rge_g,
\end{align*}
where we assume $A_N^{(k)} \neq 0$ at $q$ for $k=1,2$. Otherwise one already has $A_N^{(1)} = A_N^{(2)}$. 
To determine $A_N^{(k)}$, we follow the same argument as before.
Symmetrically, we can consider the $(2N+1)$th linearization 
\[
\partial_{\epsilon_1}\partial^{2N-2}_{\epsilon_2}\partial_{\epsilon_3}\partial_{\epsilon_4} L_{A^{(k)}, h^{(k)}}(f) |_{\epsilon_1 = \epsilon_2 = \epsilon_3 = \ep_4=0}
\]
and so on to have 
\begin{align*}
&\lge A_2^{(1)}, 8\zeta 
- 2\zeta^{(j)} \rge_g  = \lge A_2^{(2)}, 8\zeta 
- 2\zeta^{(j)} \rge_g, \quad j = 2,3,4,
\end{align*}
and when $N \geq 3$ we have
\[
\lge A_N^{(1)}, \zeta 
+\frac{1}{2N-2}   \zeta^{(j)} \rge_g  
= \lge A_N^{(2)}, \zeta 
+\frac{1}{2N-2}  \zeta^{(j)} \rge_g, \quad j = 2,3,4.
\]
A summation over $j=1,2,3,4$ shows that 
\begin{align*}
&\lge A_2^{(1)}, 30\zeta \rge_g  = \lge A_2^{(2)}, 30\zeta  \rge_g, 
\end{align*}
and 
\[
(4 + \frac{1}{2N-2})\lge A_N^{(1)}, \zeta \rge_g =(4 + \frac{1}{2N-2})\lge A_N^{(2)}, \zeta \rge_g, \quad N \geq 3.
\]
Note that $(q, \zeta)$ is regularly observable by Lemma \ref{lm_3null}. 
We can determine $\lge A_N^{(1)}, \hat{\zeta }\rge_g =\lge A_N^{(2)}, \hat{\zeta} \rge_g$ for any $\hat{\zeta} \in N^+(\zeta, \varsigma)$ with some $\varsigma >0$.   
This implies $A_N^{(1)} = A_N^{(2)}$ at $q$. 

Next, we can subtract the contribution of $\mathcal{U}^{2N+1}_{N, 0}$ from $\mathcal{U}^{2N+1}_{N}$ and compare the homogeneous term of order $\mu(2N-2,4)- 3/2$ in (\ref{ps_uNN1}) and (\ref{ps_uNN1_N2}) ({\color{Blue}or the principal symbols in (\ref{ps_uNN1_v}) and (\ref{ps_uNN1_v_N2})}) to have 
\begin{align*}
\iota \divg(A_N^{(1)}) + \sum_{\alpha+ \beta=N}\lge  A_\alpha^{(1)}, A_\beta^{(1)} \rge_g + h_{N}^{(1)}
= \iota \divg(A_N)^{(2)} + \sum_{\alpha+ \beta=N}\lge  A_\alpha^{(2)}, A_\beta^{(2)} \rge_g + h_{N}^{(2)},
\end{align*}
for $N \geq 2$.
This implies $h_{N}^{(1)} = h_{N}^{(2)}$ at $q$. 

 
%%%%%%%%%%%%%%%%%%%%% remark %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{remark}\label{rm_f4}
%    Note that we would like to choose special $v_j$ such that the only nonvanishing term is 
%    $\lge A_N, \diff( \cjv_1^{N-3} v_1^{N+1} \cjv_j \cjv_k \cjv_l) \rge $. 
%    This probably can be achieved by choosing $f_1, f_2, f_3, f_4$ by Remark \ref{rm_fj}, such that
%    \begin{itemize}
%        \item[(1)] ${\sigmp}(v_j) =  0$ near $(q, \zj)$ and
%        $ {\sigmp}(v_j)\neq 0$ near $(q, -\zj)$, for $j = 2,3,4$, 
%        {\color{Brown}
%            \item[(2)] ${\sigmp}(v_j) \neq  0$ near $(q, \zj)$ and
%            $ {\sigmp}(v_j)= 0$ near $(q, -\zj)$, for $j = 1$.}
%        %\item[(2)] 
%    \end{itemize}
%    %We emphasize that 
%\end{remark}
%%%%%%%%%%%%%%
%First we observe that each term in (\ref{eq_h1}) and (\ref{eq_h2}) gives us a distribution 
%in $I^{4\mu+(2N-3)(\mu + \frac{3}{2}) + \frac{5}{2}, -\frac{1}{2}}(\Lambda_q, \Lambda_q^g)$, 
%if we restrict them in $\nxxi$ 
%away from $\unionGamma$. 
%On the other hand, applying $Q_g$ to each term in (\ref{eq_h3}) gives us a distribution 
%in $I^{4\mu+(2N-3)(\mu + \frac{3}{2}) + \frac{3}{2}, -\frac{1}{2}}(\Lambda_q, \Lambda_q^g)$. 
%This implies terms in (\ref{eq_h1}) and (\ref{eq_h2}) contribute to the leading singularities. 
%%%%%%%%%%%%% question page %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newpage
%In particular, we choose $f_1, f_2, f_3, f_4$ as in Remark \ref{rm_f4}. 
%By (\ref{eq_psmodel}), the principal symbol of each of them at $(y,\eta)$ will vanish if $v_3$ or $v_4$ appears. 
%It follows that from (\ref{eq_h1}) and  (\ref{eq_h2}) we only have the term
%%{\color{Brown}
%%\begin{align}\label{eq_termh1}
%%Q_g(
%% \sum_{\alpha  = 1}^{N-1} \lge A_N, \diff v_1 \rge v_1^{N+1 - \alpha} \cjv_1^{\alpha-1} v_2^{\alpha-1} \cjv_2^{N-1-\alpha} 
%% \cjv_3 \cjv_4 
%%).
%%\end{align}
%%}
%\begin{align}\label{eq_termh12}
%Q_g \big(
%\lge A_N, \diff (\cjv_1^{N-3} v_1^{N+1} \cjv_j \cjv_k \cjv_l)\rge_g
%+ (\lge A_N, \diff v_1 \rge_g 
%\cjv_1^{N-3} v_1^{N}) \cjv_j \cjv_k \cjv_l
%\big).
%\end{align}
%
%Note that we have
%\begin{align*}
%&{\sigmp} \big(
%\lge A_N, \diff (\cjv_1^{N-3} v_1^{N+1} \cjv_2 \cjv_3 \cjv_4)\big)(q, \zeta) \\
%=&\lge A_N, \zeta \rge_g {\sigmp}(\cjv_1^{N-3} v_1^{N+1})(q, \zeta^{(1)})
%{\sigmp}(\cjv_2)(q, \zeta^{(2)})
%{\sigmp}(\cjv_3)(q, \zeta^{(3)})
%{\sigmp}(\cjv_4)(q, \zeta^{(4)}), \\
%%%%%%%%%%%
%&{\sigmp} \big(
%\lge A_N, \diff v_1 \rge_g 
%\cjv_1^{N-3} v_1^{N}) \cjv_j \cjv_k \cjv_l
%\big)(q, \zeta) \\
%=&{\sigmp}(\lge A_N, \diff v_1 \rge_g 
%\cjv_1^{N-3} v_1^{N})(q, \zeta^{(1)})
%{\sigmp}(\cjv_2)(q, \zeta^{(2)})
%{\sigmp}(\cjv_3)(q, \zeta^{(3)})
%{\sigmp}(\cjv_4)(q, \zeta^{(4)}).
%\end{align*}
%We can compute ${\sigmp}(\lge A_N, \diff v_1 \rge_g 
%\cjv_1^{N-3} v_1^{N})(q, \zeta^{(1)})$ by Lemma \ref{lm_product}. 
%We have
%\begin{align*}
%&{\sigmp}(\lge A_N, \diff v_1 \rge_g 
%\cjv_1^{N-3} v_1^{N})(q, \zeta^{(1)}) \\
%= & {\sigmp}( \lge A_N, \diff v_1 \rge_g)  \ast
%{\sigmp}(v_1^{N}\cjv_1^{N-3}) (q, \zeta^{(1)})  \\
%= & (\lge A_N, \eta \rge_g {\sigmp}(v_1)) \ast 
%\underbrace{{\sigmp}(v_1) \ast \ldots \ast {\sigmp}(v_1) }_{N} \ast
%\underbrace{{\sigmp}(\cjv_1) \ast \ldots \ast {\sigmp}(\cjv_1) }_{N-3} (q, \zeta^{(1)}). 
%\end{align*}
%
%
%{\color{blue} \text{Question: how do we determine $A_N$ from (\ref{eq_termh12})? }}
%\vspace{3cm}
%
%Can we choose $v_1$ such that $\overline{{\sigmp}(v_1)(q, -\zeta^{(1)})} = {\sigmp}(v_1)(q, \zeta^{(1)})$?
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%If so, then by \cite[Lemma 5.1]{Kurylev2018} , one has
%\[
%\lge A_N, \diff v_1 \rge  v_1^{N} \in \mathcal{I}^{\mu + N(\mu+\frac{3}{2}) + 1}(\Lambda_1), \quad v_2^{N-2} \in \mathcal{I}^{\mu + (N-3)(\mu+\frac{3}{2})}(\Lambda_2).
%\]
%We apply Lemma \ref{lm_fourwaves} to have 
%\begin{align*}
%\lge A_N, \diff v_1  \rge v_1^{N} \cjv_2^{N-2} \cjv_l \cjv_k  \in \mathcal{I}^{4\mu+(2N-3)(\mu + \frac{3}{2}) + \frac{5}{2}, -\frac{1}{2}}(\Lambda_q, \Lambda_q^g)
%\end{align*}
%in $\nxxi$ and away from $\unionGamma$. 
%The principal symbol at $(q, \zeta) \in \Lambda_q$ away from $\unionGamma$ is 
%\[
%{\sigmp}(\lge A_N, \diff v_1  \rge v_1^{N} \cjv_2^{N-2} \cjv_l \cjv_k) = (2\pi)^{-3}  
%\lge A_N,  {\sigmp}(v_1^{N}\diff v_1)(q, \zeta^{(1)}) \rge
%\]
%%%%%%%%%%%%% question page %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
